AttackBench: Evaluating Gradient-based Attacks for Adversarial Examples

Adversarial examples are typically optimized with gradient-based attacks. While novel attacks are continuously proposed, each is shown to outperform its predecessors using different experimental setups, hyperparameter settings, and number of forward and backward calls to the target models. This provides overly-optimistic and even biased evaluations that may unfairly favor one particular attack over the others. In this work, we aim to overcome these limitations by proposing AttackBench, i.e., the first evaluation framework that enables a fair comparison among different attacks. To this end, we first propose a categorization of gradient-based attacks, identifying their main components and differences. We then introduce our framework, which evaluates their effectiveness and efficiency. We measure these characteristics by (i) defining an optimality metric that quantifies how close an attack is to the optimal solution, and (ii) limiting the number of forward and backward queries to the model, such that all attacks are compared within a given maximum query budget. Our extensive experimental analysis compares more than $100$ attack implementations with a total of over $800$ different configurations against CIFAR-10 and ImageNet models, highlighting that only very few attacks outperform all the competing approaches. Within this analysis, we shed light on several implementation issues that prevent many attacks from finding better solutions or running at all. We release AttackBench as a publicly-available benchmark, aiming to continuously update it to include and evaluate novel gradient-based attacks for optimizing adversarial examples.

==> legacy.tex <==

\begin{comment}
\subsubsection{Initialization Strategies}
Some attacks perform a custom initialization to favor a better exploration of the loss landscape. 
Initialization can be modeled as transformations 
$i: \mathbb{R}^\con d \to \mathbb{R}^\con d$, and return a valid sample in the feasible domain.
The baseline option is to start the attack from the original point (\originalinit). 
Another option is choosing a random initialization (\randominit), which sets the initial estimate of $\vct \delta_0$ to be a random perturbation within the constraints of the optimization problem, as done by \fab~\cite{croce2020minimally}. 
Note that some attacks may also internally run the attack starting from multiple random restarts and take the best perturbation out of all trials to improve the optimization results~\cite{Croce2019SparseAI}.
Other attacks, like \bb~\cite{brendel2020accurate} and optionally \fmn~\cite{pintor2021fast}, can be initialized as a sample belonging to a specific target class (\adversarialinit), and minimize the perturbation by getting closer and closer to $\vct x$ during the iterations.

\subsubsection{Descent Directions}

To speed-up the optimization, attacks use different  strategies that modify the gradient in each iteration before passing it to the optimizer (\cref{line:gradient_transform}).
We identify four main strategies to define appropriate descent directions:

\mylist{1.} Gradient (\nochange), which uses the gradient $\vct g$ \textit{as is};

\mylist{2.}  Normalization (\normalization), which keeps the direction of $\vct g$ but rescales its norm to be proportional to the step size $\stepsize_\stepindex$ in the current iteration, \ie, $\vct g^{\prime} = \frac{\stepsize_\stepindex \vct g}{s}$, where the scaling factor is often set as $s=\| \vct g \|_p$;

\mylist{3.}  Projection (\linearproj), which sets the direction by maximizing the scalar product with the gradient $\vct g$ over an $\stepsize_\stepindex$-sized $\ell_p$ ball, as $\vct %g^{\prime} \in \underset{\parallel \vct v \parallel_p \leq \stepsize_\stepindex}{\argmax } \, \vct v^\top \vct g$;
g^{\prime} \in \argmax_{\parallel \vct v \parallel_p \leq \stepsize_\stepindex} \, \vct v^\top \vct g$;\footnote{This amounts to maximizing the linear approximation of the loss function $L(\vct x + \vct v, y, \vct \theta) \approxeq L(\vct x, y, \vct \theta) + \vct v^T \nabla L(\vct x, y, \vct \theta)$ over an $\stepsize_\stepindex$-sized $\ell_p$ ball.}

\mylist{4.} Proximal (\prox), which uses the proximal gradient~\cite{parikh2014proximal}.


PGD-based attacks all use \linearproj, as for $p \in \{1, 2, \infty\}$ the solution can be efficiently computed in closed form. 
For $p=1$, the maximum is achieved by taking the  components of $\vct g$ with maximum absolute values and setting them to $\pm \stepsize_\stepindex$, according to their sign. 
In practice, this leads to poor performance when combined with the box constraint in \cref{eq:bounds_min_distance}, as it results in updating only one component in each iteration.
Reformulations of this update generally include the box constraint in the maximization, \eg, in $\ell_1$-\apgd~\cite{croce2020reliable}, which update the components exhibiting the largest absolute values at once, up to the box limits, until an \ellone norm of $\stepsize_\stepindex$ is achieved.
For $p=2$, the maximum is achieved when $\vct g^\prime = \stepsize_\stepindex\frac{\vct g}{\|\vct g\|_2}$, which is practically equivalent to \normalization.
For $p=\infty$, the maximum is achieved by setting $g^\prime = \sign(\vct g)$, resulting in a dense update of all components of $\vct \delta_\stepindex$ as in the \ellinf-\pgd attack~\cite{madry18-iclr}. 



\subsubsection{Optimizers}
This attack component applies the update on the current perturbation, producing a new perturbation $\vct \delta_\stepindex$. 
Optimizers are specific algorithms that implement this update, $u: \mathbb{R}^\con d \mapsto \mathbb{R}^\con d$, based on the computed gradient and a specific strategy (\cref{line:opt_step}) and return a perturbation vector of the same dimension as the input . 
Existing gradient-based adversarial attacks use different variants of Gradient Descent (\GD), sometimes with a diagonal metric to scale different axes of the space (\eg Adam (\Adam)) or introducing a momentum term to avoid vanishing gradient issues (\eg Momentum (\MomentumGD)). 
Alternatively, they can use adaptive strategies where the learning rate changes over time (\eg RMSprop with momentum (\RMSPropMomentum)) or second-order derivative methods (\eg \BFGSB). Optimizers can also be combined together as in attacks that integrate linear solvers with other gradient-based sub-routine attacks (\GDLinearSolv).
Finally, the optimizer step might include a final projection operation that ensures the produced update $\vct x + \delta_\stepindex$ is in the feasible domain. 
Specifically, it takes into account the box constraint in~\cref{eq:pareto} and eventually the $\pertsize$ bound in \cref{eq:constr_max_conf} for the case of \maxloss attacks.


\subsubsection{Step Size Schedulers}
Some attacks, including most of the \maxloss attacks, use a fixed step size (\fixed).
However, as well known in optimization theory, when using \GD, decreasing the step size usually leads to better convergence results. 
Thus, dedicated schedulers can control the optimization process. We denote them as a function $h: \mathbb{R} \mapsto \mathbb{R}$, that dynamically updates the step size $\stepsize$ (\cref{line:gamma_decay}) and tune the decay to guarantee better convergence.    
Indeed, many attacks, especially the \minnorm, reduce the step size along the iterations, shrinking the trust region of the linear approximation (thus, the step size) to refine the solution with smaller updates as they approach the boundary. 
One common strategy is to use a linear step size decay (\linear), in which the step size is multiplied by a fixed amount $\gamma<1$ at each step. 
Another popular scheduler is the Cosine Annealing (\cosine)~\cite{loshchilov2017sgdr}, which decays the step size gradually from a maximum value of $\stepsize$ to a minimum of $\stepsize_\numberofsteps$. 
Other alternatives are exponential (\exponential) or polynomial (\polynomial) step size decay, where the decay is controlled by an exponential descent or a specified polynomial, respectively. 
As another strategy, some attacks adapt the step size depending on the loss behavior over a span of iterations. 
In particular, when the loss plateaus for a specified number of steps, this scheduler reduces the step size by a defined factor (\plateau).
While these attacks are often called \textit{adaptive}, the term adaptive is already used in the State of the Art of adversarial attacks for denoting attacks that are customized to break a specific defense
~\cite{tramer2020adaptive}.

% \subsection{Further Implementation Remarks}
% \myparagraph{Heuristics to improve performances.} 
% It is worth noting that some attacks use heuristics to improve the optimization results even further. 
% Firstly, some adapt the hyperparameters (\eg, the step size) to each sample individually.
% This is the case of the \cw attack, that uses a line search to find the best penalty weight per sample.
% Another example is \apgd, which uses a \plateau strategy to find the most suitable learning rate sample-wise, thus refining the results better for each individual sample.
% In contrast, others keep the same strategy across batches or even an entire dataset.
% Second, some attacks use multiple restarts to reduce the sensitivity to the initialization and further improve the results.
% Hence, they optimize adversarial examples starting for multiple initialization points, and they pick the best results across restarts.
% \mpcomment{also, APGD does a strange thing with the init, using smoothed gradient instead of the original gradient for the first step. We should be capturing this with the benchmark, right?}

% \myparagraph{Additional observations.}
% \mpcomment{I want to put here all misconceptions or observations that make the paper tutorial on adversarial examples, I think it is important to value these as well}
% First, as well known, optimization algorithms only find local solutions to the problem.
% The global minima are unknown and finding them would require conducting an exhaustive search, which is not possible in most cases.
% Thus, local solutions are accepted as an estimate of the robustness of the models, as they are  the best achievable estimate of the global solutions. 
%\mpcomment{expand this taken from intro}
%This is not a problem in general, but many works in the literature erroneously compare their efficacy without considering their different nature, thus spreading false conclusions about their performances.
%Regarding maximum confidence attacks, all the proposed evaluations keep feeding the misconception that adversarial attacks must be tested for a specific intensity of the perturbation, causing experiments conducted in research papers to overfit this setting, ignoring that robustness should be a general property of machine learning models under test
%
%\mpcomment{perhaps here we can write about attacks on other problems (\eg detection), domains, non-additive perturbations (\eg adv. malware)}



\end{comment}




==> metrics.tex <==
% \myparagraph{Query-distortion curves.} To evaluate each attack in terms of perturbation size under the same query budget $Q$, we use the so-called query-distortion curves introduced by Brendel \etal~\cite{brendel2020accurate}. These curves report, for each attack, the median value of $\vct \delta^\star$ as a function of the number of  queries $Q$. For each given $Q$ value, the optimal $\vct \delta^\star$ for each point is selected among the different attack executions (\ie using different hyperparameters and/or initialization points. 

\myparagraph{Perturbation size.} The median value of $\| \vct \delta^\star \|$ at $Q=1000$ queries (\ie the last value from the query-distortion curve), for all models, attacks and norms. 

\myparagraph{Robust accuracy.} \mpcomment{Here we write how to compute robust accuracy etc.}

\myparagraph{Convergence speed.} To get an estimate of the convergence speed, We can compare robust accuracies for different query budgets to take into account the convergence speed.

\myparagraph{Robustness to hyperparameter selection.} Selecting the optimal hyperparameters for each point is computationally demanding and rarely done in practice. It is thus of interest to evaluate how sensitive an attack is to a suboptimal selection of its hyperparameters. To this end, we optimize the hyperparameters at the dataset-level (\ie using the same configuration for all testing points) and measure the difference to the case in which they are optimized at the sample-level.

\myparagraph{Execution time.} The average runtime per query for each attack-model pair, measured on a worsktation \mpcomment{TODO}.

\myparagraph{Number of forwards/backwards.} \mpcomment{TODO}

\myparagraph{Implementation issues.} \mpcomment{ (time, CPU/GPU,...), here we write what we had to fix because some attacks have problems - like CW iterations - then we detail them in exp section or appendix} 


==> tables/attacks_summary.tex <==

\begin{table*}[!htbp]
    \centering
    \caption{List and categorization of earlier adversarial attacks, and of the attacks considered in our evaluation benchmark.}
    \label{table:adv_attacks_categorization}
     \resizebox{\textwidth}{!}{%
    \rowcolors{15}{}{gray!10}
    \begin{tabular}{lllccccllllll}
    \toprule
    \multirow{2}{*}{\textbf{Name}} & \multirow{2}{*}{\textbf{Attack Type}} & \multicolumn{4}{c}{\textbf{Norms}} & \multirow{2}{*}{\textbf{\makecell{Descent\\Direction}}} & \multirow{2}{*}{\textbf{Optimizer}} & \multirow{2}{*}{\textbf{\makecell{Step size ($\alpha$)\\ Scheduler}}}   & \multirow{2}{*}{\textbf{Loss} $L$} & \multirow{2}{*}{\textbf{Init} $\delta_0$}\\
     & & \multicolumn{1}{c}{$\ell_0$} & $\ell_1$ & $\ell_2$ & $\ell_\infty$ & &  & &  & \\
    \midrule
    \biggio~\cite{biggio13-ecml} (2013) & \maxloss &  & \multicolumn{1}{c}{\tcheck} & \multicolumn{1}{c}{\tcheck} & \multicolumn{1}{l}{} & \nochange & \GD & \fixed & $f_y(\vct x; \vct \theta)$ & \originalinit \\
    \szegedy~\cite{szegedy14-iclr-intriguing} (2014) & \minnorm & & &  \multicolumn{1}{c}{}  & \multicolumn{1}{l}{\tcheck} & \nochange & \BFGSB  & \fixed & \crossentropy & \originalinit \\
    \fgsm~\cite{goodfellow15-iclr-explaining} (2015) & \maxloss &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{c}{\tcheck} & $\linearproj$ & \GD & \fixed & \crossentropy & \originalinit \\ \midrule
    %
    \jsma~\cite{papernot16-sp} (2015) & \minnorm & \multicolumn{1}{c}{\tcheck} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & $\linearproj$ & \MomentumGD & \fixed & $z_y(\vct x; \vct \theta)$  & \originalinit \\
    %
    \bim~\cite{kurakin16adversarialexamples} (2016) & \maxloss &  &  &  & \tcheck & \linearproj & \GD & \fixed & \crossentropy & \originalinit \\
    %
    \dfool~\cite{moosavi16-deepfool} (2016) & \minnorm &  &  & \tcheck & & \normalization & \GD & \fixed & \logitloss & \originalinit \\
    %
    \cw~\cite{carlini17-sp} (2017) & \minnorm & \tcheck &  & \tcheck & \tcheck & \nochange & \Adam & \fixed & \logitloss & \originalinit  \\
    %
    \ead~\cite{chen2018ead} (2018) & \minnorm &  & \tcheck & \tcheck & \tcheck & \nochange & \GD & \polynomial & \logitloss & \originalinit  \\
    %
    \pgd~\cite{madry18-iclr} (2018) & \maxloss &  &  & \tcheck & \tcheck & \linearproj & \GD & \fixed & \crossentropy & \originalinit \\
    %
    \bb~\cite{brendel2020accurate} (2019) & \minnorm & \tcheck & \tcheck & \tcheck & \tcheck & \linearproj & \BFGSB & \linear & \logitloss & \adversarialinit \\
    %
    \ddn~\cite{rony2019decoupling} (2019) & \minnorm  &  & & \tcheck & & \normalization & \GD & \cosine & \crossentropy & \originalinit \\
    %
    \pgdlzero~\cite{Croce2019SparseAI} (2019) & \maxloss  & \tcheck &  & &  & \linearproj & \GD & \fixed & \crossentropy & \originalinit \\
    %
    \sfool~\cite{Modas2018SparseFoolAF} (2019) & \minnorm &  & \tcheck & & & \normalization & \texttt{GD$^\star$} & \fixed & \logitloss & \adversarialinit \\
    %
    \tr~\cite{Yao2018TrustRB} (2019) & \minnorm &  & \multicolumn{1}{l}{} & \tcheck & \tcheck & \nochange & \GD & \fixed & \logitloss & \originalinit \\
    %
    \fab~\cite{croce2020minimally} (2020) & \minnorm  &  & \tcheck & \tcheck & \tcheck & \linearproj & \GD & \plateau & \logitloss & \randominit \\
    %
    \apgd~\cite{croce2020reliable} (2020) & \maxloss  &  &  & \tcheck & \tcheck & \linearproj & \MomentumGD & \plateau & \crossentropy/\dlr & \originalinit \\
    %
     \alma~\cite{Rony2020AugmentedLA} (2021) & \minnorm  &  & \tcheck & \tcheck & \multicolumn{1}{l}{} & \nochange & \RMSPropMomentum & \exponential & \dlr & \originalinit  \\
    %
    \apgdlone~\cite{Croce2021MindTB} (2021) & \maxloss  &  & \tcheck &  &  & \linearproj & \MomentumGD & \plateau & \dlr & \originalinit \\ 
    %
    \fmn~\cite{pintor2021fast} (2021) & \minnorm  & \tcheck & \tcheck & \tcheck & \tcheck & \normalization & \GD & \cosine & \logitloss & \anyinit \\
    %
     \pdgd~\cite{Matyasko2021PDPGDPP} (2021) & \minnorm & & & \tcheck & & \linearproj & \Adam & \linear, \exponential & \logitloss & \originalinit \\
    %
     \pdpgd~\cite{Matyasko2021PDPGDPP} (2021) & \minnorm & \multicolumn{1}{c}{\tcheck} & \tcheck & \tcheck & \tcheck & \prox & \Adam & \linear, \exponential & \logitloss & \originalinit \\
    %
    \vfga~\cite{Hajri2020StochasticSA} (2021) & \minnorm  & \multicolumn{1}{c}{\tcheck} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \nochange & \texttt{GD$^\star$} & \fixed & $z_y(\vct x; \vct \theta)$  & \originalinit   \\ 
    %
    \sigmazero~\cite{Cina2024SigmaZero} (2024) & \minnorm  & \multicolumn{1}{c}{\tcheck} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \normalization & \Adam & \cosine & \logitloss & \originalinit   \\ \bottomrule
    \end{tabular}
    }
    \end{table*}

==> unified_algorithm.tex <==
\begin{algorithm}[t]
 \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwComment{Comment}{$\triangleright$\ }{}
    \DontPrintSemicolon
	\caption{Generalized Attack Algorithm}
	\label{algo:unified_attack_algorithm}
   \Input{$\vct x$, the input sample; $y$, the class label; \stepsize, the initial step size; $\vct \theta$, target model; and \numberofsteps, the number of iterations.}
	\Output{The adversarial example $\vct x_{\rm adv}$.}
     $\vct \delta_{0} \gets \textcolor{orange}{\texttt{init}}(\vct x) $\label{line:init}\Comment*[r]
     {\textcolor{orange}{initialization}}
    $\vct \delta^\star \gets \vct \delta_0$, $\alpha_{0}=\alpha$ \\
    \For {$\stepindex = 1, \ldots, \numberofsteps$} 
	    {$\vct g \gets \nabla_{\vct \delta} \textcolor{blue}{L}(\vct x +\vct \delta_{k-1}, y,  \vct \theta)$ \Comment*[r]{\textcolor{blue}{loss} gradient}\label{line:gradient}
    $\vct g \gets \textcolor{violet}{\texttt{direction}}(\vct g, \stepsize_\stepindex)$\label{line:gradient_transform}\Comment*[r]{\textcolor{violet}{descent direction}}
        $\vct \delta_{k} \gets$ \textcolor{cyan}{\texttt{optim}}($\vct x, \vct \delta_{k-1}, \vct g)$ \label{line:opt_step} \Comment*[r]{\textcolor{cyan}{optimizer} (proj.)}
        %$\vct \delta_{k} \gets \vct \delta_{k-1} -  \Pi_{\alpha_k}(\vct g)$ \\
        %$\Pi(\vct x +\vct \delta_k) $ \\
        
	   $\stepsize_{\stepindex} \gets \textcolor{red}{\texttt{scheduler}}(\stepsize_{0}, \stepindex, \numberofsteps)$ \Comment*[r]{\textcolor{red}{scheduler}} \label{line:gamma_decay}
        %$\alpha_{\stepindex} \gets \gamma_\stepindex \alpha$ \Comment*[r]{scheduler step}\label{line:step_decay}
        %$\vct \delta_k \gets \Pi_\Delta (\vct x_0, \vct \delta_k)$ \label{line:project} \Comment*[r]{projection onto $\Delta$}
    }

 $\vct \delta^\star \gets \texttt{best}(\vct \delta_0, ... \vct \delta_\numberofsteps$)\label{line:return} \Comment*[r]{best solution}
	\bfseries return $\vct x_{\rm adv} = \vct x + \vct \delta^\star$ 
\end{algorithm}
